Public Information Representation for Adversarial Team Games

The peculiarity of adversarial team games resides in the asymmetric information available to the team members during the play, which makes the equilibrium computation problem hard even with zero-sum payoffs. The algorithms available in the literature work with implicit representations of the strategy space and mainly resort to Linear Programming and column generation techniques to enlarge incrementally the strategy space. Such representations prevent the adoption of standard tools such as abstraction generation, game solving, and subgame solving, which demonstrated to be crucial when solving huge, real-world two-player zero-sum games. Differently from these works, we answer the question of whether there is any suitable game representation enabling the adoption of those tools. In particular, our algorithms convert a sequential team game with adversaries to a classical two-player zero-sum game. In this converted game, the team is transformed into a single coordinator player who only knows information common to the whole team and prescribes to the players an action for any possible private state. Interestingly, we show that our game is more expressive than the original extensive-form game as any state/action abstraction of the extensive-form game can be captured by our representation, while the reverse does not hold. Due to the NP-hard nature of the problem, the resulting Public Team game may be exponentially larger than the original one. To limit this explosion, we provide three algorithms, each returning an information-lossless abstraction that dramatically reduces the size of the tree. These abstractions can be produced without generating the original game tree. Finally, we show the effectiveness of the proposed approach by presenting experimental results on Kuhn and Leduc Poker games, obtained by applying state-of-art algorithms for two-player zero-sum games on the converted games

==> content/1_introduction.tex <==
\section{Introduction}\label{sec:intro}
% team problem importance
Research efforts on imperfect information games customarily focus on two-player zero-sum (we refer to these games with ``2p0s'' from here on) scenarios, in which two agents act on the same environment, receiving opposite payoffs. In this setting, superhuman performances have been achieved even in large instances of games, such as \textit{Poker Hold'em} by \cite{BrownS17,Brown885,Moravck2017DeepStackEA}, and \textit{Starcraft II} by \cite{Vinyals2019GrandmasterLI}.
%
%On the other hand, autonomous agents are increasingly employed in many different contexts. This raises the issue of designing techniques to produce robust agents also in the case in which multiple agents act in the same environment, possibly sharing their rewards.
%
The customary approach for 2p0s games is based on the generation of a game abstraction that is used offline to find a  blueprint strategy which is refined online during the play.
%
Instead, the problem of solving  games with multiple players is far from being addressed and lacks of  well-assessed techniques.


In this work, we focus on adversarial team games in which a team of two (or more) agents cooperates against a common adversary. In particular, we focus on the \textit{ex ante coordination} scenario in which the team members agree on a common strategy beforehand and commit to play it during the game, without communicating any further. Examples of such a scenario are collusion in poker games, the defenders in the card-playing stage of \textit{Bridge}, and a team of drones acting against an adversary. Technically speaking, the team members share the same payoffs and coordinate against an adversary having opposite payoffs, in face of private  information given separately to each team member.

% history of the field
A natural way to characterize the desired behavior by each agent is the  \textit{team-maxmin} equilibrium (TME) solution concept, defined by Von Stengel in \cite{VonStengelKoller97}. In \cite{Celli2018ComputationalRF}, this concept is extended to extensive-form games considering different means of communication. The team-maxmin equilibrium with correlation (TMECor) characterizes optimal rational behavior in the \emph{ex ante} coordination scenario we consider in this paper. While the existance and uniqueness of value of a TMECor is guaranteed, the computation of an equilibrium corresponding to this solution concept is proven to be an inapproximable, \textsf{NP}-hard problem \cite{Celli2018ComputationalRF}. Therefore, the main open challenge is to efficiently find a strategy profile corresponding to a TMECor in a generic adversarial team game.

%%% --- maybe move to a related works section with the public infomation stuff from Nayyar and Forester?
% current approaches
\textbf{Related works.} %Classical algorithms already developed for 2p0s games cannot be applied directly to team games since the private information held by each team member cannot be shared with the other team members; therefore the problem of finding a TMECor in an adversarial team game has been customarily addressed through the design of \textit{ad hoc} techniques. 
The approaches available in the literature to solve adversarial team games mainly resort to  mathematical programming or reinforcement learning tools.

Mathematical programming approaches are generally based on \textit{column generation}. They constrain the team to play a probability distribution over a finite set of correlated plans, and iteratively add new correlated plans giving the maximum increase in value for the team. % until no new plans can be added. 
% The constraint to draw plans from a finite set for the team 
This constraint allows a polynomial-time formulation of the TMECor problem, while the plan to add is determined by using an oracle working in an implicit formulation of the normal-form representation of the original game in which the private information of a team player can be ignored during the selection of a plan. \textit{Hybrid Column Generation} (HCG)~\cite{Celli2018ComputationalRF} iteratively solves two linear programs to determine the TMECor strategy profile of the team and the adversary considering the limited set of plans available, while uses a integer linear program to find the best response joint plan to add to the currently considered plans given the current strategy of the adversary. \textit{Fictitious Team Play} (FTP)~\cite{Farina2018ExAC} is instead a \textit{fictitious play}~\cite{BrownFP} procedure running on a modified representation of the original game; in this representation one of the two team members selects a pure strategy at the start of the game, while the other team member plays against the adversary in the original game considering his teammate fixed as specified by their chosen plan. \textit{Faster Column Generation} (FCG)~\cite{Farina2021ConnectingOE} is a column generation algorithm similar to HCG, but working in a more efficient semi-randomized correlated plans representation, prescribing a pure strategy for one team member and a mixed strategy for the other. This representation also allows a cost-minimizing formulation of the best response problem as a dual of the program to find a TMECor considering the restricted set of plans. Overall, those procedures are general and simple to implement, but the use of linear programs strongly limits the scalability of these exact formulations.

Multi-Agent Reinforcement learning (MARL) approaches avoid considering plans over the entire game, and instead explicitly model the correlating coordination signal in the original extensive form adversarial team game. \textit{Soft Team Actor-Critic} (STAC)~\cite{Celli2019CoordinationIA} fixes a number of possible uniform signals at the start of the game and uses a modified actor-critic procedure to converge to a strategy for each player for each signal. \textit{Signal Mediated Strategies} (SIMS)~\cite{Cacciamani2021MultiAgentCI} works in a \textit{perfect-recall refinement} of the original game, populates a buffer of trajectories sampled from the optimal strategy for the joint team against the adversary in this refined game, and learns a distributed strategy for each team member in the original game from the trajectories in this buffer. Overall, RL techniques are more scalable than the mathematical programming ones, but present convergence issues. Indeed, STAC does not have any guarantees of converging to an equilibrium, while SIMS is guaranteed to converge only on a particular class of Adversarial Team Games.
%%% --- 

The above approaches work with an implicit strategy space representation that does not allow the adoption of standard abstraction algorithms. 
Even more in general, the problem of identifying a suitable strategy representation over which generating abstractions is open with these games.


% my contributions
\textbf{Original contributions.} We propose an algorithmic procedure, called \algoname{PublicTeamConversion}, to convert a generic instance of a team game into a 2p0s game, and provide three pruning techniques to reduce the size of the converted game. Our conversion enables the adoption of customary techniques for automated abstractions, game solving and online strategy refinement.
%
We formally prove that a Nash Equilibrium in the converted game corresponds to a TMECor in the original game. In addition, we present vEFG, an alternative description of extensive-form games better suited for the characterization of public information.

% The core idea of our approach is to combine the sharing of all team members' strategies with the use of public information to determine a belief over the possible private information of all team members.  As the game progresses, the information state of each player is enriched by the notion that other team members may or may not be in a specific private state given the deterministic strategy shared at the start of the game and the observed public actions played. In fact, playing a specific action when the overall strategy is known, communicates part of the private information.  Following this intuition, we propose an explicit representation for the game by joining the team members into a single coordinator who has an information state based only on the public information shared among team members and that prescribes a deterministic action for each possible private state of the player.
% \textcolor{red}{SCRIVERE FORNIAMO PROVE ALTERNATIVE CHE IN ALCUNI GIOCHI IL PROBLEMA E' POLINOMIALE IN QUANTO L'ALBERO PRODOTTO E PRUNATO E' POLINOMIALE} \textcolor{blue}{Dove lo facciamo?}

% related works
Our work builds upon Nayyar et al. in \cite{Nayyar2013DecentralizedSC}; similarly to our work, a shared coordinator, living in the public information state of the team, prescribes an action to the team members for any possible private state allowing the training of a common strategy for the team.  This coordinator-based transformation is recently employed in the fully cooperative setting of \textit{Hanabi} \cite{Foerster2019BayesianAD,Sokota2021SolvingCG}. However, their transformation applies to the context of decentralized stochastic control in a fully cooperative scenario, whereas we generalize such coordinator transformation in an adversarial team game setting.


==> content/2_preliminaries.tex <==
\section{Preliminaries}\label{sec:prelimi}
In this section, we provide a formal introduction to the notation used in the paper, mainly derived from the one presented in \cite{Kovarik_Schmid_Burch_Bowling_Lisy_2020}, and define the crucial concepts of Nash Equilibrium and TMECor.

%efg
An \textit{extensive form game with imperfect information} (EFG) $\mathcal G$ is a tree model representing a sequential finite interaction among different players, obtaining a payoff at the end of each trajectory of play. 
The \textit{set of players} is $\mathcal N = \{1,\dots,N\}$, and we use $c$ to indicate the \textit{chance player}. The chance player represents Nature in the game, and plays a fixed strategy $\sigma_c$.
Given a player $p$, we use $-p$ to indicate all the players different from $p$, chance included.
The \textit{action set} is indicated as $\mathcal A = \bigcup_{p \in \mathcal N} \mathcal A_p$, and each node $h$ of the tree is identified by the tuple of actions played to reach this point of the game, called \textit{history}. 
Similarly, the \textit{set of histories} is denoted by  $\mathcal H = \bigcup_{p \in \mathcal N} \mathcal H_p$. 
Given two histories $h,g$ we indicate with $h \sqsubset g$ if $h$ is a parent history of $g$. 
$\mathcal Z = \{h \in \mathcal H : \not \exists g, h \sqsubseteq g \}$ is the set of \textit{terminal histories}, also called leaf histories, and $u_p(z): \mathcal Z \to \mathbb{R}$ is the utility of player $p$ upon reaching terminal history $z$. 
$\mathcal N(h)$ and $\mathcal A(h)$ indicate respectively the player playing and the actions available to play in node $h$. $ha$ indicates the history reached by playing action $a$ in $h$.
To indicate the information state of a player $p$, we define $\mathcal I_p$ as a partition over $\mathcal H_p$, indicating the nodes which are indistinguishable for a player. $I \in \mathcal I_p$ is called \textit{information set} and we have the constraint that $\forall h,h' \in I : \mathcal A(h) = \mathcal A(h')$. We use $\mathcal A(I)$ to indicate the actions available in a information state and $\mathcal I(h)$ to indicate the information set of a history.

% behavioral strategies and normal form plans
In this setting, we have different options to represent a strategy of each player. 
A \textit{behavioral strategy} $\sigma_p(I): \mathcal I_p \to \Delta^{|A(I)|}$ is a function associating to each information set of player $p$ a probability distribution over the possible actions.
A \textit{normal form plan} (also called plan or pure strategy) $\pi_p \in \Pi_p := \bigtimes_{I \in \mathcal I_p} \mathcal A(I)$ for player $p$ is a tuple specifying an action for each information set of $p$. A \textit{normal form strategy} $\mu_p \in \Delta^{|\Pi_p|}$ is a probability distribution over plans.

% perfect recall & timeability
An EFG has \textit{perfect recall} if for every $p \in \mathcal N$, for every $I \in \mathcal I_i$ and any pair $h, h' \in I$, the sequences of infosets and actions of player $p$ leading to $h, h'$ are the same.

For a EFG, a deterministic timing is a labelling of the nodes in $\mathcal H$ with non-negative real
numbers such that the label of any node is at least one higher than the label of its parent. A deterministic timing is exact if any two nodes in the same information set have the same label. A EFG is \textit{timeable} if it admits a deterministic exact timing. A EFG is \textit{1-timeable} if it admits a deterministic exact timing such that each node's label is exactly one higher than its parent's label.

% \begin{lemma}[Equivalence of timeable and 1-timeable EFGs \cite{Kovarik_Schmid_Burch_Bowling_Lisy_2020}]
% Any classical timeable EFG can be made 1-timeable by adding chance nodes with a single noop action. This modification will not increase the size of the game more than quadratically.
% \end{lemma}

A \textit{strategy profile} is a tuple associating a strategy with each player. The expected value for a player can be defined as $u_p(\boldsymbol{\sigma}) = u_p(\sigma_p, \boldsymbol{\sigma_{-p}}) = \sum_{z \in \mathcal Z} \rho^{\boldsymbol{\sigma}}(z) u_p(z)$, where $\rho^{\boldsymbol{\sigma}}(z)$ indicates the probability of reaching terminal node $z$ given the strategies of all players.
%
%payoff equivalence
Any two strategies of a player are called \textit{payoff equivalent} if, for any strategy of the other players, both strategies have the same expected payoff.
%
Given a player $p$ and a strategy for all the other players $\boldsymbol{\sigma_{-p}}$, a \textit{best response strategy} $BR(\boldsymbol{\sigma_{-p}})$ for $p$ is a strategy maximizing their expected payoff.
%
% Nash Equilibrium
A \textit{Nash Equilibrium} (NE) is a strategy profile $\boldsymbol \sigma$ such that no player can gain a larger payoff value by deviating to a different strategy. Formally, $\forall p \in \mathcal N : \sigma_p \in BR(\boldsymbol{\sigma_{-p}})$
%
% TMECor
A \textit{Team Maxmin equilibrium with correlation} (TMECor) is a TME equilibrium in which all team players are correlated. Formally, a TMECor is a strategy profile $\boldsymbol \sigma^*$ such that: 
$\boldsymbol \sigma^* = \argmax_{\boldsymbol{\sigma_{\mathcal T}} \in \Delta^{|\bigtimes_{p \in \mathcal T} \Sigma_p|}} \min_{\sigma_o} u_{\mathcal T}(\boldsymbol{\sigma_{\mathcal T}}, \sigma_o)$

% % two player zero sum games
% A game is said to be \textit{two-player zero-sum} (2p0s) if it has two players only and any gain from one player is a cost for the opponent.

% % common payoff game
% A game is said to be \textit{common payoff} if all the players share the same utility function.

% % adversarial team game
% A game is said to be an \textit{adversarial team game} (ATG) if it has at least three players, and its player set is partitioned into a single player called opponent and a set called team, such that team players all share the same utility function which is the opposite of the opponent's.
\fe{Questa sezione va aggiustata, introdurre formalmente adversarial team games e sistemare il resto}

==> content/2_preliminaries_1.tex <==
\section{Preliminaries}\label{sec:prelim}
%
In this section, we introduce the basic concepts and definitions that we need throughout this work (for more details, we refer the interested reader to \cite{shoham-leyton}).
%
\paragraph{Extensive-Form Games and Adversarial Team Games}

The basic model for sequential interactions among a set $\mathcal{N}$ of multiple agents with private information is the \emph{Extensive-Form Game with imperfect information} (EFG). 
%
If chance is present in the game we enrich the set of players with the chance player $c$ and chance probabilities are denoted as $\sigma_c$. 
%
An EFG defines a tree where the set of nodes is denoted by $\mathcal{H}$ and the leaves (terminal nodes of the game) are denoted by $\mathcal{Z}\subseteq\mathcal{H}$. 
%
The player that acts at a node $h\in\mathcal{H}$ is identified by the function $\mathcal{P}(h) \in \mathcal{N}$, and the set of actions that she can choose at $h$ are $A(h)$.
%
Let $u_p: \mathcal{Z}\to\Reals$ be the payoff function of player $p$ that maps every terminal node to an utility value.
%
In order to account for imperfect information, we use \emph{information sets} (infosets).
%
An infoset $I\subseteq\mathcal{H}$ is a partition of the nodes of the tree in which a player acts such that they are indistinguishable to her. 
%
We denote the set of player $p$ infosets as $\mathcal{I}_p$.
%
With a slight abuse of notation, we indicate the player that acts at infoset $I$ as $\mathcal{P}(I)$ and her available actions at that infoset as $A(I)$.
%
Furthermore, the action space is defined as $\mathcal{A} = \bigcup_{p\in\mathcal{N}}\mathcal{A}_p$, where $\mathcal{A}_p = \bigcup_{I\in\mathcal{I}_p} A(I)$.
%
In this work we are interested in Adversarial Team Games (ATG).
%
An ATG is a $N$ player EFG in which there is a \emph{team} $\mathcal{T}\subseteq\mathcal{N}$ of players that plays against a single opponent ($\mathcal{N} = \mathcal{T}\cup\left\{ o\right\}$, where $o$ is the opponent). 
%
Here, the team is represented by a set of agents that share the same utility function.
%
Formally $\forall p \in \mathcal{T}$, $u_p = u_\mathcal{T}$ for some function $u_\mathcal{T}$. 
%
We restrict our analysis to zero-sum ATG, i.e., games in which $u_{\mathcal{T}} = -u_o$.
%
For a EFG, a deterministic timing is a labelling of the nodes in $\mathcal{H}$ with non-negative real
numbers such that the label of any node is at least one higher than the label of its parent. 
%
A deterministic timing is exact if any two nodes in the same information set have the same label. 
%
A EFG is \emph{1-timeable} if it admits a deterministic exact timing such that each node's label is exactly one higher than its parent's label.
%
Furthermore, we require that all the players involved in the game have the property of \emph{perfect recall}, \emph{i.e.,} they never forget information they previously knew during the game.

\paragraph{Strategies and Nash Equilibrium}
%
There are several possible ways of representing strategies in these classes of games. 
%
A \emph{behavioral strategy} $\sigma_p: \mathcal{I}_p\to\Delta^{|A(I)|}$ is a function that maps each infoset to a probability distribution over available actions. 
%
A \emph{normal-form plan} (or \emph{pure strategy}) $\pi_p\in\Pi_p:= \bigtimes_{I\in\mathcal{I}_p}A(I)$ is a tuple specifying one action for each infoset, while a \emph{normal-form strategy} $\mu_p\in\Delta^{|\Pi_p|}$ is a probability distribution over normal-form plans. 
%
With a slight abuse of notation, $\forall p \in\mathcal{N}$ we write with $\sigma_p[z]$ (respectively $\mu_p[z]$) the probability of reaching terminal node $z\in\Z$ when following strategy $\sigma_p$ (resp. $\mu_p$). 
%
A strategy profile is a tuple associating a strategy to each player in the game. 
%
We denote normal-form strategy profiles as $\boldsymbol{\mu}$ and behavioral strategy profiles as $\boldsymbol{\pi}$. 
%
Given a strategy profile $\boldsymbol{\mu}$, we denote with $\mu_p$ the strategy of player $p\in\N$ and with $\boldsymbol{\mu}_{-p}$ the strategies of all the other players. 
%
With an abuse of notation, the expected utility for player $p$ when she plays strategy $\mu_p$ and all the other players play strategy $\boldsymbol{\mu}_{-p}$ is $u_p(\mu_p, \boldsymbol{\mu}_{-p})$.
%
Furthermore, we define the \emph{best response} of player $p$ to strategy profile $\boldsymbol{\mu}_{-p}$ as the strategy that maximizes player $p$'s utility against strategy $\boldsymbol{\mu}_{-p}$.
%
Formally, $BR_p(\boldsymbol{\mu}_{-p}) := \argmax_{\mu} u_p(\mu, \boldsymbol{\mu}_{-p})$.
%
A strategy profile $\boldsymbol{\mu}$ is a Nash Equilirbium (NE) if it is stable to respect to unilateral deviations of a single player. 
%
Formally, $\boldsymbol{\mu}$ is a NE if and only if $\forall p \in \mathcal{N}$, $\mu_p \in BR_p(\boldsymbol{\mu}_p)$.

% \fe{Cambiare la notazione ? ($\sigma$ per la forma normale, $\pi$ per la behavioral)}


==> content/3_tmecor.tex <==
\section{How to Enforce Coordination Between Team Members}\label{sec:tmecor}

When considering ATGs, the problem of computing optimal strategies for the team of agents becomes inherently more complex. 
%
This happens because, in order to maximize their utility, the team players need to coordinate their strategies. 
%
In practice, such a requirement on coordination is translated into the formulation of an \emph{ad-hoc} solution concept for Adversarial Team Games. 
%
Von Stengel and Koller, in \cite{VonStengelKoller97}, introduce the \emph{Team Maxmin Equilibrium} (TME), that is defined as the NE in which the team's utility is maximized. 
%
The solution concept described by the TME exhibits some appealing characteristics: (i) in some cases it can be arbitrarily more efficient in terms of payoffs for the team with respect to a NE, (ii) it is unique (except for degeneracies), thus it does not suffer from equilibrium selection issues \cite{Basilico2016teammaxmin,Basilico2017ComputingTT,Celli2018ComputationalRF}.
%
However, it is not easy to be computed as it does not admit a convex mathematical formulation \cite{Farina2021ConnectingOE}.

If the coordination of team's strategies is done \emph{ex-ante}\footnote{Note that different form of coordination are possible, (\emph{e.g.,} intra-play) but they require communication capabilities between the team members that are not allowed in general games.} (\emph{i.e.,} before the beginning of each game), it is possible to introduce a new solution concept, called \emph{Team Maxmin Equilibrium with a Correlation device} (TMEcor) \cite{Celli2018ComputationalRF}. 
%
Such a coordination has the advantage to increase the expected utility of the team \cite{Celli2018ComputationalRF}. Moreover, differently than the TME, the TMEcor can be computed through a Linear Program that considers joint normal-form plans of the team players: 
%
\begin{equation}\label{eq:tmecor}
\begin{array}{l}\displaystyle
\max_{\mu_\team}\min_{\mu_o} \sum_{z\in\Z}\hspace{.4cm} \mu_\team[z]\,\mu_o[z]\,u_\team(z)\\
\hspace{.3cm}\textnormal{s.t. }\hspace{.5cm}\mu_\team\in\Delta(\bigtimes\limits_{p\in\team}\Pi_p)\\[4mm]
\hspace{1.3cm}\mu_o\in\Delta(\Pi_o)
\end{array}
\end{equation}
%

In general, the dimension of the strategy space of the team $\bigtimes_{p\in\team} \Pi_p$ grows exponentially in the number of team members, thus increasing the complexity of solving the LP in Equation~\eqref{eq:tmecor}.
%
sThere are, however, some specific cases in which it is possible to compute or approximate efficiently the TMEcor, simply by considering all the team members as a unique meta-player $\team$ and applying state-of-the-art algorithms for finding NE in 2p0s games.
%
In order to use these techniques, it is necessary that the meta-player has perfect recall. 
%
The requirement of perfect recall for the team is satisfied only when the information available to the team players is symmetric, (\emph{i.e.,} they all observe something or none of them does).
%
Unfortunately, this is not usually the case. 
%
In principle, the sources of imperfect recall for the team can be different\footnote{We refer the interested reader to the appendix for a more detailed description of the aforementioned cases.
}: (i) non-visibility over a team member's action, (ii) non-visible game structure, (iii) private information disclosed only to a subset of team members. % \fe{Metterei in appendice la sezione che aveva scritto precedentemente Luca}
%
Mathematical programming algorithms \cite{Celli2018ComputationalRF,Farina2018ExAC,Farina2021ConnectingOE}  address the problem of imperfect recall for the team by considering the space of joint strategies. When the support of the TMEcor strategy for the team is small, they can efficiently converge to the equilibrium.
%
On the other hand, MARL solutions, like SIMS \cite{Cacciamani2021MultiAgentCI}, are capable of solving case (i), but fail to deal with the other sources of imperfect recall.
%
In this work, exploiting the concept of public information, we introduce a method that allows us to deal with all the three sources of imperfect recallness, opening to the possibility of using state-of-the-art RL algorithms (e.g., Deep-CFR\cite{Brown2019DeepCR}) to solve ATGs.
%
We do this first by defining a game formalism that enriches EFGs with information on public observability of actions, and then by formulating a method that transforms the original ATG into an equivalent 2p0s EFG. 

==> content/3_vefg_repr.tex <==
\section{vEFG Representation}\label{sec:vefg}
Characterizing the public information for a set of players is not possible with the standard EFG notation, since the information structure is solely defined by its information set partitions, and it is difficult to determine common patterns in the partitions of multiple players. In this section, we therefore introduce a refined formalization derived from EFGs called \textit{extensive form games with visibility} (vEFG). A vEFG is identical to an EFG, apart from the introduction of an explicit visibility function $Pub_p(a)$, describing whether an action is detected by player $p$ or not. The information state of a player in a history is determined by considering the actions of that history that are visible to him. This allows to make the information known to a player more explicit than in traditional EFGs.

The \textit{visibility function} is formally defined as $Pub_p(a): \mathcal A \to \{\mathrm{seen,unseen}\}$.
 
% Some properties of the visibility function are specified:
A vEFG has \textit{perfect recall} if any action played by a player is seen by the player himself. 
% for each non terminal history, we expect all actions to have the same visibility. This last constraint is a logical constraint not impacting the expressive power of the model, but allowing a more explicit information representation. Note that such a constraint may at most double the size of the game with respect to the original EFG version. This can intuitively be proven by decomposing each node into a series of actions that communicate to the players whether or not they will see the final action chosen.
%$$\forall h \in H, \forall p \in \mathcal N, \exists v \in \{\mathrm{seen}, \mathrm{unseen}\}, \forall a \in \mathcal A(h) : Pub_p(a) = v$$ 

The visibility function can also be extended to sets of players. $Pub_A(a): \mathcal A \to \{\mathrm{pub,priv,hidden}\}$, such that: 
\begin{align*}
& Pub_A(a) = \mathrm{pub} \iff \forall p \in A:Pub(a)=\mathrm{seen}\\
& Pub_A(a) = \mathrm{hidden} \iff \forall p \in A:Pub_p(a) = \mathrm{unseen}\\
& Pub_A(a) = \mathrm{priv} \text{ otherwise}
\end{align*}

From the visibility function it is then possible to derive the classical information set structures and the notion of public tree.

The information set structure $\mathcal I = (\mathcal I_p)_{p\in\mathcal N}$ can be recovered from $Pub_p$, by considering in the same infoset the histories corresponding to the same sequence of seen actions from a player. Formally, $\forall h,h' \in \mathcal H : h,h' \in I \subset \mathcal I_p$ if and only if $\mathcal N(h) = \mathcal N(h') = p$ and $(a)_{a\in h : Pub_p(a)=\text{seen}} = (a')_{a'\in h' : Pub_p(a')=\text{seen}}$ 
% \begin{align*}
% & \mathcal N(h) = \mathcal N(h') = p\\
% & \text{and}\\
% & (a)_{a\in h : Pub_p(a)=\text{seen}} = (a')_{a'\in h' : Pub_p(a')=\text{seen}}
% \end{align*}

$\mathcal S$ is the \textit{public tree} associated to the game. $S\in \mathcal S$ is called \textit{public state}. Two histories belong to the same public state if they share the same public actions (considering every player) and differ only by the private actions. Formally, $h,h'$ belong to the same public state iff ${(a)_{a\in h : Pub_{\mathcal N}(a)=\mathrm{pub}} = (a')_{a'\in h' : Pub_{\mathcal N}(a')=\mathrm{pub}}}$. We also use $\mathcal S(h)$ to indicate the public state associated to a history.
Moreover, we can also define the public tree for a subset of players. Given a subset of players $X \subset \mathcal N$, then $\mathcal S_X$ is the public tree associated to players in X.

We conjecture that the set of vEFGs with perfect recall is equivalent to the set of EFGs with perfect recall. Note that in vEFG we have no notion of forgetting actions, thus imperfect recall situations in which an observation is forgotten by a player cannot be represented.

In order to guarantee a specific structure of the vEFGs we treat, we introduce the concept of \textit{public turn-taking}, characterizing games in which the sequence of players acting is common knowledge across all players. Intuitively, each player knows when other players played an action in the past, even if the game has imperfect information and the specific action played may be hidden. This is a refinement to the concept of 1-timeability, in which not only the length of the history is identical but also the sequence of players.

\begin{definition}[Public turn-taking property]
A vEFG is public turn-taking if:
\begin{equation*}
\forall I \in \mathcal I, \forall h,h' \in I : (\mathcal P(g))_{g \sqsubseteq h} = (\mathcal P(g'))_{g' \sqsubseteq h'}
\end{equation*}
\end{definition}

\begin{lemma}[Transformation into public turn-taking game]
Any vEFG can be made public turn-taking by adding player nodes with a single noop action. This modification will not increase the size of the game by a factor larger than $(|\mathcal N| + 1)|\mathcal H|^2$.
\label{le:turnTaking}
\end{lemma}


==> content/3_vefg_repr_1.tex <==
\section{vEFG Representation}\label{sec:vefg}
%
In this section we introduce the concept of \emph{Extensive Form Game with visibility} (vEFG), a game formulation that overcomes the limits of EFGs, allowing the characterization of the information common to a set of players.
%
The vEFG is an EFG enriched with a visibility function $Pub_p(a): \mathcal{A}\to\{\text{seen},\text{unseen}\}$ that specifies wether an action $a\in\mathcal{A}$ performed by any player  has been observed by player $p$.
%
With an abuse of notation we define the $Pub$ function also for a set of players $\mathcal{P}\subseteq\mathcal{N}$.
%
Formally, $Pub_{\mathcal{P}}: \mathcal{A}\to\{\text{pub},\text{priv},\text{hidden}\}$ such that:
%
\begin{align*}
& Pub_{\mathcal{P}}(a) = \mathrm{pub} \iff \forall p \in \mathcal{P}:Pub_p(a)=\mathrm{seen}\\
& Pub_{\mathcal{P}}(a) = \mathrm{hidden} \iff \forall p \in \mathcal{P}:Pub_p(a) = \mathrm{unseen}\\
& Pub_{\mathcal{P}}(a) = \mathrm{priv} \text{ otherwise}.
\end{align*}

The game tree $\St$ associated to the vEFG is called \emph{public tree}.
%
A state $S\in\St$ is called \emph{public state}.
%
Two game histories belong to the same public state if they share the same public actions and differ only by their private actions. 
%
Formally, $h,h'$ belong to the same public state if and only if ${(a)_{a\in h : Pub_{\mathcal N}(a)=\mathrm{pub}} = (a')_{a'\in h' : Pub_{\mathcal N}(a')=\mathrm{pub}}}$.
%
We also use $\St(h)$ to indicate the public state associated to a history $h$.
%
Moreover, given a subset of players $X \subset \mathcal N$, we can define the public tree for $X$ as $\St_X$ such that ${(a)_{a\in h : Pub_{X}(a)=\mathrm{pub}} = (a')_{a'\in h' : Pub_{X}(a')=\mathrm{pub}}}$.

The information set structure $\mathcal I = (\mathcal I_p)_{p\in\mathcal N}$ can be recovered from $Pub_p$, by considering in the same infoset the histories corresponding to the same sequence of seen actions from a player.
%
Formally, $\forall h,h' \in \mathcal H : h,h' \in I \subset \mathcal I_p$ if and only if $\mathcal P(h) = \mathcal P(h') = p$ and $(a)_{a\in h : Pub_p(a)=\text{seen}} = (a')_{a'\in h' : Pub_p(a')=\text{seen}}$.

% \ma{in che senso? Lo proviamo?}We conjecture that the set of vEFGs with perfect recall is equivalent to the set of EFGs with perfect recall. 
%
Note that in vEFGs we have no notion of forgetting actions, thus imperfect recall situations in which an observation is forgotten by a player cannot be represented.

As the only assumption for our method, we restrict the class of games we consider, introducing the concept of \textit{public turn-taking}.
%
This concept characterizes games in which the sequence of acting players is common knowledge across all players. 
%
Intuitively, each player knows when other players played an action in the past, even if the game has imperfect information and the specific action played may be hidden. 
%
This is a refinement to the concept of 1-timeability, in which not only the length of the history is identical but also the sequence of players.
%
\begin{definition}[Public turn-taking property]
A vEFG is public turn-taking if:
\begin{equation*}
\forall I \in \mathcal I, \forall h,h' \in I : (\mathcal P(g))_{g \sqsubseteq h} = (\mathcal P(g'))_{g' \sqsubseteq h'}
\end{equation*}
\end{definition}
%
\begin{theorem}[Transformation into public turn-taking game]
Any vEFG can be made public turn-taking by adding player nodes with a single noop action. The size of the resulting game tree is $(|\mathcal N| + 1)|\mathcal H|^2$.
\label{le:turnTaking}
\end{theorem}


==> content/4_info_structure.tex <==
\section{Information Structure in Team Games}\label{sec:info_struct}
The core problem of finding a TMECor in adversarial team games resides in \textit{asymmetric visibility}, since team members have a private state that does not allow to create a joint coordination player.

In the following we characterize the possible types of asymmetric visibility that may cause imperfect recall for the joint player, and singularly address them.

\textbf{Non-visibility over a team member's action}. If a team member plays a action which is hidden from another team member, the joint team player would have imperfect recall due to forgetting his own played actions. This source of imperfect recallness can be avoided in a TMECor by considering the shared deterministic strategies before the game starts. This allows to know a priori which are the exact actions played by team members in each node. Thus it is safe to apply a perfect recall refinement in the original game, which corresponds to always consider the chosen action of a team member as $\mathrm{seen}$ by other team members.

\textbf{Non-visible game structure}. Consider two nodes in the same information set for a player before which the other team member may have played a variable number of times, due to a chance outcome non visible to the team member of this nodes. In this case a perfect recall refinement is not applicable to distinguish the nodes, because it would give the joint coordinator a visibility not correspondent to the one of the players in the game. To solve this edge case, we require the property of public turn-taking.

\textbf{Private information disclosed by chance/adversary to specific team members.} It is the most complex type of non visibility, since in a TMECor we have no explicit communication channels through which share information, and therefore this type of joint imperfect recall can only be addressed by considering a strategically equivalent representation of the game in which at most one of the team players has private information. 
%In fact, this specific type of non visibility is the one avoided by SIMS, since no perfect recall refinement can perform such a transformation, and solved through the normal form representation of a team player in HCG, FTP, FCG, since the choice of a plan is independent of the private information discovered during the game.

State of the art techniques address this issue by considering a richer representation of the original game, to make more explicit the information needed for an effective team coordination.

\textit{Linear programming} (LP) approaches use a normal form representation for one or both the team members. This because a normal form plan allows one to specify the complete strategy of a player in one shot, and by sharing this information with the other team member (or equivalently, by correlating each player's plan selection), they can optimize their strategy knowing how the other member will behave for the rest of the game. This solves the coordination problem, at the cost of large action space for the normalized players.

\textit{Reinforcement learning} (RL) approaches work on a refined representation of the original game, without any normalization. This avoids the exponential growth of the size of the game representation. However, such game representation lacks enough information to fully characterize the coordination among team members. In the case of STAC, the fragmented and fixed system of signals severely affects the convergence performances, while SIMS guarantees convergence only on instances without private observations, which is not the case of most practical team coordination problems.

The main theoretical advance of the present work is the use of a transformation based on public information of the team to solve this problem of private information.

Our \algoname{PublicTeamConversion} transformation builds upon the one proposed by \cite{Nayyar2013DecentralizedSC}. The main idea is to substitute team players in the original game with a coordinator that only sees public information among team members. The coordinator prescribes the action of the currently playing team member by emitting a prescription directed to them, associating each possible private state of the player with one possible action. In this way, each player becomes a \textit{puppet agent} which executes the prescriptions received by using the private information at his disposal. The important feature is that such a coordinator only lives in the space of public information of the team, and therefore the decision points giving prescriptions to each team player can be associated to a unique player.

Intuitively, we can see this process of prescription as a weak normalization. In fact, we maintain the public tree structure of the original game, while we normalize each public state, in the sense that we build smaller local plans with an action for each private state corresponding to a public state. As in the normal form conversion, we still have an exponential explosion due to the combination of actions for each private state, but the decomposition per public state makes it more computationally tractable, especially when employing pruning techniques.


==> content/5_public_conversion.tex <==
\section{Public Team Conversion Algorithm}\label{sec:conversion}
%By combining the various solutions proposed for the different types of private information, we can formulate a conversion procedure able to convert an adversarial team game into a 2p0s game, in which a coordinator player takes the strategic decision in behalf of the team.
We present the algorithmic procedure to convert an adversarial team game into a 2p0s game, in which a coordinator player takes the strategic decision on behalf of the team. The pseudo-code is shown in ~\cref{alg:PubTeam}.

The algorithm recursively traverses the original game tree in a post-order depth-first fashion: for each traversed node, corresponding nodes are instantiated in the converted game. The chance, terminal, and adversary nodes are copied unaltered since the coordinator player $t$ has only access to the public information visible to the team members. 
%
Each team member node is instead mapped to a new coordinator node, in which he plays a prescription $\Gamma$ among the combination of possible actions for each information state $I$ belonging to the public team state. % of the node to convert. 
%
Given a public state $S$, the coordinator issues to the players different recommendations for every possible information set belonging to $S$.
%
As an example, consider to be in a state of the original game in which one of the team players has to choose between actions $\mathcal{A} = \{a_1,...,a_n\}$ and that her private state can be either $S_1$ or $S_2$. 
% 
Then, the recommendation issued by the coordinator is a tuple that specifies one action for each possible private state (\emph{e.g.,} a valid recommendation would be to play action $a_i$ when the private state is $S_1$ and to play action $a_j$ when the private state is $S_2$).
Once the original ATG has been transformed into a 2p0s game, we can solve the latter with state-of-the-art algorithm for this class of games (\emph{e.g.,} CFR, CFR+, MCCFR, DeepCFR).
%
We show an example of a two players team game and its converted game in~\cref{app:figures}. 
%3
To ease the visualization, we focus on a cooperative game with no adversary.

%
The following Theorem constitutes the main result of this work.
%
It shows the equivalence between a NE of the converted 2p0s game and a TMEcor of the original ATG, thus enabling the usage of a powerful set of tools to compute equilibria for ATGs. 
%
\begin{theorem} \label{th:main}
Given a public-turn-taking vEFG $\mathcal G$, and the correspondent converted game $\mathcal G' = \algoname{ConvertGame}(\mathcal G)$, a Nash Equilibrium in $\mathcal G'$ corresponds to a TMECor in $\mathcal G$.
\end{theorem}
%
The proof is in~\cref{app:proofs}. 

\begin{algorithm}[!htb]
\caption{Public Team Conversion}\label{alg:PubTeam}
\begin{algorithmic}[1]
	\Function {ConvertGame}{$\mathcal G$}
		\State initialize $\mathcal G'$ new game
		\State $\mathcal N' \gets \{t,o\}$
		\State $h'_{\emptyset} \gets$ \Call{PubTeamConv}{$h_{\emptyset}, \mathcal G, \mathcal G'$} \Comment{new game root}
		\State \Return{$\mathcal G'$}
	\EndFunction
	\item[] % to skip line
	\Function{PubTeamConv}{$h$, $\mathcal G$, $\mathcal G'$}
		\State initialize $h' \in \mathcal H'$
  		\If {$h \in \mathcal Z$} \Comment{terminal node}
  			\State $h' \gets h' \in \mathcal Z'$
  			\State $u'_p(h') \gets u_p(h) \quad \forall p \in \mathcal N$
  		\ElsIf {$\mathcal P(h) \in \{o, c\}$} \Comment{opponent or chance}
  			\State $\mathcal P'(h') \gets \mathcal P(h)$
  			\State $\mathcal A'(h') \gets \mathcal A(h)$
  			\If {$h$ is chance node}
  				\State $\sigma_c'(h') = \sigma_c(h)$
  			\EndIf
  			\For {$a' \in \mathcal A'(h')$}
  				\State $Pub_t'(a') \gets$ check $Pub_{\mathcal T}(a') = \mathrm{pub}$
  				\State $Pub_o'(a') \gets Pub_o(a')$
  				\State $h'a' \gets$ \Call{PubTeamConv}{$ha'$, $\mathcal G$, $\mathcal G'$}
  			\EndFor 
  		\Else \Comment{team member}
  			\State $\mathcal P'(h') = t$
  			\State $\mathcal A'(h') \gets \bigtimes_{I \in \mathcal  S_{\mathcal T}(h)} \mathcal A(I)$ \Comment{prescriptions}
  			\For {$\Gamma' \in \mathcal A'(h')$}
  				\State $Pub_t'(\Gamma') \gets \mathrm{seen}, Pub_o'(\Gamma') \gets \mathrm{unseen}$
  				\State $a' \gets \Gamma'[\mathcal I(h)]$ \Comment{extract chosen action}
  				\State initialize $h'' \in \mathcal H'$
  				\State $\mathcal A'(h'') \gets \{a'\}$
 				\State $\mathcal P(h'') = c$
  				\State $Pub_t'(a') \gets \mathrm{seen}$
 				\State $Pub_o'(a') = Pub_o(a')$
 				\State $\sigma_c'(h'') =$ play $a'$ with probability 1
  				\State $h''a' \gets$ \Call{PubTeamConv}{$ha'$, $\mathcal G$, $\mathcal G'$}
  				\State $h'\Gamma \gets h''$ 
  			\EndFor 
  		\EndIf
  		\State \Return $h'$
	\EndFunction
\end{algorithmic}
\end{algorithm}



==> content/6_pruning.tex <==
\section{Pruning techniques}\label{sec:pruning}

The conversion procedure presented is important to prove the equivalence between the original team game and its converted version, but it is not enough for practical applications. 
In fact, applying \cref{alg:PubTeam} to a public state in the original game with $A$ actions for $S$ possible private states results into $A^S$ prescriptions, producing a tree with an exponentially large fan-out.
% While the computation of a TMECor has a unavoidable exponential complexity due to the \textsf{NP}-hardness of the problem\ma{CITA}, any 2p0s solving algorithm can strongly benefit of any improvement made to the game size. 
We propose three pruning techniques to attenuate the computational challenges of the converted game allowing the application of existing algorithms for equilibrium learning or computation.

\textbf{Pruned Representation}. 
Whenever a prescription is issued to a team member that has to play a public action, the played action can be used to exclude the private states for which a different action has been given. 
%
This practice allows us to safely exclude a subset of the possible private states reducing the number of possible prescriptions in successive nodes.
%
% This pruning effect is particularly effective when the chosen prescriptions are various, suggesting many different actions; on the other hand, non informative prescriptions associating the same action to all private states do not allow the exclusion of any private state.


\textbf{Folding Representation}. Consider the case of the extraction of a specific chance outcome when this is a private information for a team member and unseen by the adversary (e.g. a private card in poker). We can avoid to add this node to the converted game, and instead maintain the probability that each player is in a specific private state, given that some may be excluded as in the pruned representation. Then we modify the chance node $h''$ after each prescription to sample an action according to the sum of the probabilities of the private states for which that action has been prescribed.
%In the original game, chance outcomes are explicitly represented independently by the visibility of the outcomes, branching the game tree in different subgames according to the specific outcome. Consider the case of the extraction of a specific outcome when this is a private information for a team member and unseen by the adversary. In the converted game, such a outcome is not visible to any player, and can therefore be safely postponed as long as no specific action depends on it. The folding representation takes advantage of this property to avoid sampling these types of private state, and instead sampling an action from the prescription depending on the probability (also called belief) that in a certain point in the game a specific private state is present given the previous actions of all players. The dummy chance nodes $h''$ instantiated in Algorithm \ref{alg:PubTeam} therefore may present different actions each with a probability that is the sum of the probability of the private states for which that action has been prescribed. This representation also takes advantage of the computed beliefs to reduce the prescriptions given by the coordinator as in the pruning representation.
%
Overall, the game size is reduced in case many private states for the players are sampled. Such a representation is similar to the public belief state representation proposed in \cite{Brown_Bakhtin_Lerer_Gong_2020}. The name folding representation derives from the fact that trajectories with same public actions but different private states are folded one over the other in the converted game.

\textbf{Safe Imperfect Recallness}. 
%
Whenever a team player is in a state with three or more actions available, a specific action is played and some possible private states are excluded from the belief. 
%
The specific actions prescribed for the excluded states are not important to describe the information state of the player; we can therefore forget part of the prescription and have imperfect recall among different prescriptions with different prescribed actions for excluded states. 
%
While this pruning technique does not directly reduce the number of nodes, it reduces the number of information sets, simplifying the information structure of the game. 
%
This reduces the space requirements to represent the strategies, and makes the algorithms converge faster. 
%
This pruning technique is theoretically sound, and the convergence properties of CFR in this imperfect recall setting have already been addressed by \cite{Lanctot_Gibson_Burch_Zinkevich_Bowling_2012}.

Examples of the pruning techniques described are shown in Appendix~\ref{app:figures}. 

==> content/7_experiments.tex <==
\section{Experiments}\label{sec:experiments}
In this section, we evaluate the benefits of the pruning techniques when applied to a toy game, and  present the application of our conversion procedure to multiplayer instances of Kuhn and Leduc poker.
%
Details on the experimental setting and further experimental results are shown in the Appendix.
%
\subsection{Impact of Pruning techniques}
To evaluate the impact of pruning techniques, we designed a simple parametric game for which we are able to determine in closed-form the total number of nodes.
%
For the sake of simplicity, we can ignore the presence of an opponent (recall that opponent and chance nodes are copied as they are, hence they do not have an impact on the increase in size of the converted game).
%
The game we considered is a two player game $\mathcal G$, with players $P1$ and $P2$, in which there are $C$ chance outcomes at root, observed by $P1$ and not by $P2$. 
%
After observing the outcome of the chance node, $P1$ acts sequentially $H$ times, each time choosing between $A$ actions.
%
$P2$ does not observe the actions performed by $P1$. 
%
Finally, at the last round of the game, $P2$ acts, choosing between $A$ actions. 

We evaluate the size of the games obtained by applying the basic algorithm and the sizes of the games obtained through the pruning techniques presented in Section~\ref{sec:pruning} and denoted as \emph{pruning} and \emph{folding}. 
%
Furthermore, as a baseline, we show the number of normal-form plans. 
% 
Table~\ref{fig:pruning} shows the results for $C=3$, $A = 2$ and for various values of the parameter $H$.
%
The derivation of the equation that shows the total number of nodes is shown in Appendix~\ref{app:pruning}.


\begin{table*}[!ht]
\begin{subtable}{.5\textwidth}
  \input{tables/C=3, A=2, P1 only private state}
  \caption{only $P1$ has private information}
  \label{fig:sub1}
\end{subtable}
\begin{subtable}{.5\textwidth}
  \input{tables/C=3, A=2, P1 and P2 private state}
  \caption{both $P1$ and $P2$ have private information}
  \label{fig:sub2}
\end{subtable}
\caption{Comparison of total number of nodes for $C=3$, $A=2$.}
\label{fig:pruning}
\end{table*}

\begin{figure*}[!ht]
\centering
\begin{subfigure}{.47\textwidth}
  \centering
  \includegraphics[width=\textwidth]{images/Kuhn_LCFR+_np3_nc4_nr1_a0.pdf}
  
  \small{Peak RAM occupation: 96 MB}
  \caption{3-player Kuhn poker, with 4 card ranks and adversary playing first.}
  \label{fig:poker1}
\end{subfigure}%
\hspace*{0.04\textwidth}%
\begin{subfigure}{.47\textwidth}
  \centering
  \includegraphics[width=\textwidth]{images/Leduc_LCFR+_np3_nc3_nr1_a0.pdf}
  
  \small{Peak RAM occupation: 912 MB}
  \caption{3-player Leduc poker, with 3 card ranks, 1 raise, and adversary playing first.}
  \label{fig:poker2}
\end{subfigure}
\caption{Performances of Linear CFR+ applied to Poker game instances.}
\end{figure*}
% comment
We observe that pruning technique is particularly effective at dampening the exponential factor due to the combinatorial structure of prescriptions, thanks to the belief-based pruning.

Moreover, folding technique combines the benefits of the pruning technique, with the specific tradeoff imposed by the use of delayed chances. 
%
Indeed, all the histories belonging to the same public state are represented in a single node, at the cost of a chance node added after each prescription. 
%
This tradeoff is useful for game states in which many private states are possible. 
%
On the other hand, when the possible private states are reduced to one or two, the extra chance nodes added are increasing the size of the game tree more than in the pruning representation.
%
% We decide to use the folding representation as our focus in poker instances with an information structure similar to Table \ref{fig:sub2}. \fe{In che senso?}


\subsection{Application to team poker}
To test the effectiveness of our approach in a real case, we apply our conversion procedure to the multiplayer versions of Kuhn poker and Leduc poker. 
%
The Kuhn instances we use are parametric in the number of ranks available, and on whether the adversary plays first, second or third in the game. 
%
Similarly, Leduc instances are parametric on the number of ranks, on the position of the adversary, but also on the number of raises that can be made.
%
Figure~\ref{fig:poker1} and Figure~\ref{fig:poker2} show the convergence performances on the converted games of Linear CFR+ \cite{Brown2019SolvingIG}. 
%
We report a paired plot showing both the value and exploitability convergence, along with the optimal value of a TMECor as computed by \cite{Farina2021ConnectingOE}, represented as horizontal dashed lines in the team value plot.
%
The results are coherent with the theoretical result of Theorem~\ref{th:main}; the Nash Equilibrium returned by the algorithm has the same value of the TMECor of the original game.
%
We implemented the converted games in Open Spiel~\cite{lanctot2019openspiel}, taking advantage of the already available 2p0s solvers.
%
More details regarding the experimental setting are available in Appendix \ref{app:exp}, while Appendix \ref{app:sizes} shows the sizes of the converted games for a varying number of ranks and raises.
%

==> content/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
	\item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{}
\end{enumerate}

\end{enumerate}

==> content/content-aamas/2_preliminaries.tex <==
\section{Preliminaries}\label{sec:prelimi}
In this section, we provide a formal introduction to the notation used in the paper, mainly derived from the one presented in \cite{Kovarik_Schmid_Burch_Bowling_Lisy_2020}, and define the crucial concepts of Nash Equilibrium and TMECor.

%efg
An \textit{extensive form game with imperfect information} (EFG) $\mathcal G$ is a tree model representing a sequential finite interaction among different players, obtaining a payoff at the end of each trajectory of play. 
The \textit{set of players} is $\mathcal N = \{1,\dots,N\}$, and we use $c$ to indicate the \textit{chance player}. The chance player represents Nature in the game, and plays a fixed strategy $\sigma_c$.
Given a player $p$, we use $-p$ to indicate all the players different from $p$, chance included.
The \textit{action set} is indicated as $\mathcal A = \bigcup_{p \in \mathcal N} \mathcal A_p$, and each node $h$ of the tree is identified by the tuple of actions played to reach this point of the game, called \textit{history}. 
Similarly, the \textit{set of histories} is denoted by  $\mathcal H = \bigcup_{p \in \mathcal N} \mathcal H_p$. 
Given two histories $h,g$ we indicate with $h \sqsubset g$ if $h$ is a parent history of $g$. 
$\mathcal Z = \{h \in \mathcal H : \not \exists g, h \sqsubseteq g \}$ is the set of \textit{terminal histories}, also called leaf histories, and $u_p(z): \mathcal Z \to \mathbb{R}$ is the utility of player $p$ upon reaching terminal history $z$. 
$\mathcal N(h)$ and $\mathcal A(h)$ indicate respectively the player playing and the actions available to play in node $h$. $ha$ indicates the history reached by playing action $a$ in $h$.
To indicate the information state of a player $p$, we define $\mathcal I_p$ as a partition over $\mathcal H_p$, indicating the nodes which are indistinguishable for a player. $I \in \mathcal I_p$ is called \textit{information set} and we have the constraint that $\forall h,h' \in I : \mathcal A(h) = \mathcal A(h')$. We use $\mathcal A(I)$ to indicate the actions available in a information state and $\mathcal I(h)$ to indicate the information set of a history.

% behavioral strategies and normal form plans
In this setting, we have different options to represent a strategy of each player. 
A \textit{behavioral strategy} $\sigma_p(I): \mathcal I_p \to \Delta^{|A(I)|}$ is a function associating to each information set of player $p$ a probability distribution over the possible actions.
A \textit{normal form plan} (also called plan or pure strategy) $\pi_p \in \Pi_p := \bigtimes_{I \in \mathcal I_p} \mathcal A(I)$ for player $p$ is a tuple specifying an action for each information set of $p$. A \textit{normal form strategy} $\mu_p \in \Delta^{|\Pi_p|}$ is a probability distribution over plans.

% perfect recall & timeability
An EFG has \textit{perfect recall} if for every $p \in \mathcal N$, for every $I \in \mathcal I_i$ and any pair $h, h' \in I$, the sequences of infosets and actions of player $p$ leading to $h, h'$ are the same.

For a EFG, a deterministic timing is a labelling of the nodes in $\mathcal H$ with non-negative real
numbers such that the label of any node is at least one higher than the label of its parent. A deterministic timing is exact if any two nodes in the same information set have the same label. A EFG is \textit{timeable} if it admits a deterministic exact timing. A EFG is \textit{1-timeable} if it admits a deterministic exact timing such that each node's label is exactly one higher than its parent's label.

% \begin{lemma}[Equivalence of timeable and 1-timeable EFGs \cite{Kovarik_Schmid_Burch_Bowling_Lisy_2020}]
% Any classical timeable EFG can be made 1-timeable by adding chance nodes with a single noop action. This modification will not increase the size of the game more than quadratically.
% \end{lemma}

A \textit{strategy profile} is a tuple associating a strategy with each player. The expected value for a player can be defined as $u_p(\boldsymbol{\sigma}) = u_p(\sigma_p, \boldsymbol{\sigma_{-p}}) = \sum_{z \in \mathcal Z} \rho^{\boldsymbol{\sigma}}(z) u_p(z)$, where $\rho^{\boldsymbol{\sigma}}(z)$ indicates the probability of reaching terminal node $z$ given the strategies of all players.
%
%payoff equivalence
Any two strategies of a player are called \textit{payoff equivalent} if, for any strategy of the other players, both strategies have the same expected payoff.
%
Given a player $p$ and a strategy for all the other players $\boldsymbol{\sigma_{-p}}$, a \textit{best response strategy} $BR(\boldsymbol{\sigma_{-p}})$ for $p$ is a strategy maximizing their expected payoff.
%
% Nash Equilibrium
A \textit{Nash Equilibrium} (NE) is a strategy profile $\boldsymbol \sigma$ such that no player can gain a larger payoff value by deviating to a different strategy. Formally, $\forall p \in \mathcal N : \sigma_p \in BR(\boldsymbol{\sigma_{-p}})$
%
% TMECor
A \textit{Team Maxmin equilibrium with correlation} (TMECor) is a TME equilibrium in which all team players are correlated. Formally, a TMECor is a strategy profile $\boldsymbol \sigma^*$ such that: 
$\boldsymbol \sigma^* = \argmax_{\boldsymbol{\sigma_{\mathcal T}} \in \Delta^{|\bigtimes_{p \in \mathcal T} \Sigma_p|}} \min_{\sigma_o} u_{\mathcal T}(\boldsymbol{\sigma_{\mathcal T}}, \sigma_o)$

% % two player zero sum games
% A game is said to be \textit{two-player zero-sum} (2p0s) if it has two players only and any gain from one player is a cost for the opponent.

% % common payoff game
% A game is said to be \textit{common payoff} if all the players share the same utility function.

% % adversarial team game
% A game is said to be an \textit{adversarial team game} (ATG) if it has at least three players, and its player set is partitioned into a single player called opponent and a set called team, such that team players all share the same utility function which is the opposite of the opponent's.
\fe{Questa sezione va aggiustata, introdurre formalmente adversarial team games e sistemare il resto}

==> content/content-aamas/3_vefg_repr.tex <==
\section{vEFG Representation}\label{sec:vefg}
Characterizing the public information for a set of players is not possible with the standard EFG notation, since the information structure is solely defined by its information set partitions, and it is difficult to determine common patterns in the partitions of multiple players. In this section, we therefore introduce a refined formalization derived from EFGs called \textit{extensive form games with visibility} (vEFG). A vEFG is identical to an EFG, apart from the introduction of an explicit visibility function $Pub_p(a)$, describing whether an action is detected by player $p$ or not. The information state of a player in a history is determined by considering the actions of that history that are visible to him. This allows to make the information known to a player more explicit than in traditional EFGs.

The \textit{visibility function} is formally defined as $Pub_p(a): \mathcal A \to \{\mathrm{seen,unseen}\}$.
 
% Some properties of the visibility function are specified:
A vEFG has \textit{perfect recall} if any action played by a player is seen by the player himself. 
% for each non terminal history, we expect all actions to have the same visibility. This last constraint is a logical constraint not impacting the expressive power of the model, but allowing a more explicit information representation. Note that such a constraint may at most double the size of the game with respect to the original EFG version. This can intuitively be proven by decomposing each node into a series of actions that communicate to the players whether or not they will see the final action chosen.
%$$\forall h \in H, \forall p \in \mathcal N, \exists v \in \{\mathrm{seen}, \mathrm{unseen}\}, \forall a \in \mathcal A(h) : Pub_p(a) = v$$ 

The visibility function can also be extended to sets of players. $Pub_A(a): \mathcal A \to \{\mathrm{pub,priv,hidden}\}$, such that: 
\begin{align*}
& Pub_A(a) = \mathrm{pub} \iff \forall p \in A:Pub(a)=\mathrm{seen}\\
& Pub_A(a) = \mathrm{hidden} \iff \forall p \in A:Pub_p(a) = \mathrm{unseen}\\
& Pub_A(a) = \mathrm{priv} \text{ otherwise}
\end{align*}

From the visibility function it is then possible to derive the classical information set structures and the notion of public tree.

The information set structure $\mathcal I = (\mathcal I_p)_{p\in\mathcal N}$ can be recovered from $Pub_p$, by considering in the same infoset the histories corresponding to the same sequence of seen actions from a player. Formally, $\forall h,h' \in \mathcal H : h,h' \in I \subset \mathcal I_p$ if and only if $\mathcal N(h) = \mathcal N(h') = p$ and $(a)_{a\in h : Pub_p(a)=\text{seen}} = (a')_{a'\in h' : Pub_p(a')=\text{seen}}$ 
% \begin{align*}
% & \mathcal N(h) = \mathcal N(h') = p\\
% & \text{and}\\
% & (a)_{a\in h : Pub_p(a)=\text{seen}} = (a')_{a'\in h' : Pub_p(a')=\text{seen}}
% \end{align*}

$\mathcal S$ is the \textit{public tree} associated to the game. $S\in \mathcal S$ is called \textit{public state}. Two histories belong to the same public state if they share the same public actions (considering every player) and differ only by the private actions. Formally, $h,h'$ belong to the same public state iff ${(a)_{a\in h : Pub_{\mathcal N}(a)=\mathrm{pub}} = (a')_{a'\in h' : Pub_{\mathcal N}(a')=\mathrm{pub}}}$. We also use $\mathcal S(h)$ to indicate the public state associated to a history.
Moreover, we can also define the public tree for a subset of players. Given a subset of players $X \subset \mathcal N$, then $\mathcal S_X$ is the public tree associated to players in X.

We conjecture that the set of vEFGs with perfect recall is equivalent to the set of EFGs with perfect recall. Note that in vEFG we have no notion of forgetting actions, thus imperfect recall situations in which an observation is forgotten by a player cannot be represented.

In order to guarantee a specific structure of the vEFGs we treat, we introduce the concept of \textit{public turn-taking}, characterizing games in which the sequence of players acting is common knowledge across all players. Intuitively, each player knows when other players played an action in the past, even if the game has imperfect information and the specific action played may be hidden. This is a refinement to the concept of 1-timeability, in which not only the length of the history is identical but also the sequence of players.

\begin{definition}[Public turn-taking property]
A vEFG is public turn-taking if:
\begin{equation*}
\forall I \in \mathcal I, \forall h,h' \in I : (\mathcal P(g))_{g \sqsubseteq h} = (\mathcal P(g'))_{g' \sqsubseteq h'}
\end{equation*}
\end{definition}

\begin{lemma}[Transformation into public turn-taking game]
Any vEFG can be made public turn-taking by adding player nodes with a single noop action. This modification will not increase the size of the game by a factor larger than $(|\mathcal N| + 1)|\mathcal H|^2$.
\label{le:turnTaking}
\end{lemma}


==> content/content-aamas/4_info_structure.tex <==
\section{Information Structure in Team Games}\label{sec:info_struct}
The core problem of finding a TMECor in adversarial team games resides in \textit{asymmetric visibility}, since team members have a private state that does not allow to create a joint coordination player.

In the following we characterize the possible types of asymmetric visibility that may cause imperfect recall for the joint player, and singularly address them.

\textbf{Non-visibility over a team member's action}. If a team member plays a action which is hidden from another team member, the joint team player would have imperfect recall due to forgetting his own played actions. This source of imperfect recallness can be avoided in a TMECor by considering the shared deterministic strategies before the game starts. This allows to know a priori which are the exact actions played by team members in each node. Thus it is safe to apply a perfect recall refinement in the original game, which corresponds to always consider the chosen action of a team member as $\mathrm{seen}$ by other team members.

\textbf{Non-visible game structure}. Consider two nodes in the same information set for a player before which the other team member may have played a variable number of times, due to a chance outcome non visible to the team member of this nodes. In this case a perfect recall refinement is not applicable to distinguish the nodes, because it would give the joint coordinator a visibility not correspondent to the one of the players in the game. To solve this edge case, we require the property of public turn-taking.

\textbf{Private information disclosed by chance/adversary to specific team members.} It is the most complex type of non visibility, since in a TMECor we have no explicit communication channels through which share information, and therefore this type of joint imperfect recall can only be addressed by considering a strategically equivalent representation of the game in which at most one of the team players has private information. 
%In fact, this specific type of non visibility is the one avoided by SIMS, since no perfect recall refinement can perform such a transformation, and solved through the normal form representation of a team player in HCG, FTP, FCG, since the choice of a plan is independent of the private information discovered during the game.

State of the art techniques address this issue by considering a richer representation of the original game, to make more explicit the information needed for an effective team coordination.

\textit{Linear programming} (LP) approaches use a normal form representation for one or both the team members. This because a normal form plan allows one to specify the complete strategy of a player in one shot, and by sharing this information with the other team member (or equivalently, by correlating each player's plan selection), they can optimize their strategy knowing how the other member will behave for the rest of the game. This solves the coordination problem, at the cost of large action space for the normalized players.

\textit{Reinforcement learning} (RL) approaches work on a refined representation of the original game, without any normalization. This avoids the exponential growth of the size of the game representation. However, such game representation lacks enough information to fully characterize the coordination among team members. In the case of STAC, the fragmented and fixed system of signals severely affects the convergence performances, while SIMS guarantees convergence only on instances without private observations, which is not the case of most practical team coordination problems.

The main theoretical advance of the present work is the use of a transformation based on public information of the team to solve this problem of private information.

Our \algoname{PublicTeamConversion} transformation builds upon the one proposed by \cite{Nayyar2013DecentralizedSC}. The main idea is to substitute team players in the original game with a coordinator that only sees public information among team members. The coordinator prescribes the action of the currently playing team member by emitting a prescription directed to them, associating each possible private state of the player with one possible action. In this way, each player becomes a \textit{puppet agent} which executes the prescriptions received by using the private information at his disposal. The important feature is that such a coordinator only lives in the space of public information of the team, and therefore the decision points giving prescriptions to each team player can be associated to a unique player.

Intuitively, we can see this process of prescription as a weak normalization. In fact, we maintain the public tree structure of the original game, while we normalize each public state, in the sense that we build smaller local plans with an action for each private state corresponding to a public state. As in the normal form conversion, we still have an exponential explosion due to the combination of actions for each private state, but the decomposition per public state makes it more computationally tractable, especially when employing pruning techniques.


==> content/content-aamas/7_expressivity.tex <==
\section{Expressive Power and Abstractions}

\begin{figure*}[!ht]
\centering
\begin{subfigure}{.47\textwidth}
  \centering
  \includegraphics[scale=0.9]{images/simple_game.pdf}
  \caption{Example of game, limited to its first level. Player 1 and Player 2 are in the same team and have different visibility over the chance outcome. We use ``\dots'' to denote that the game can continue below.}
  \label{fig:simple_game}
\end{subfigure}%
\hspace*{0.04\textwidth}%
\begin{subfigure}{.47\textwidth}
  \centering
  \includegraphics[scale=0.9]{images/simple_game_converted.pdf}
  \caption{The corresponding converted game.}
  \label{fig:simple_game_converted}
\end{subfigure}
\caption{Example of game conversion.}
\label{fig:simple_example}
\end{figure*}

In this section, we compare the expressiveness of our converted game w.r.t. to the original extensive-form representation.

While adversary and chance players have an identical information structure as in the original game, the converted game presents a richer information structure for what concerns the team players. 
%
The use of a shared coordinator strategy allows the players to know the exact action played by their teammates for any of their private information states. This is similar to performing an \textit{inflation} \cite{Kaneko1995BehaviorSM} on the original game, recovering the extra information given to the players thanks to the property that, through \emph{ex-ante} coordination, they know the action played by their teammates in each information set.

Our converted game serves the same purpose as the \textit{Auxiliary game} introduced in \cite{Farina2018ExAC}. The goal is the same: explicitly representing the initial coordination between team members to address the imperfect recallness when representing the team as a unique player. 
%
However, in our case, the coordinator gives local prescriptions instead of the complete \emph{ex-ante} plan coordination of \cite{Farina2018ExAC}. 
%
This approach has multiple advantages:
\begin{itemize}
    \item the extensive-form representation is more efficient than the normal form with respect to the size of the resulting game \cite{Stengel1997ComputingNF}. Our converted representation takes advantage of this issue and resulting in the use of a more tractable game tree if compared to the one obtained from the normal form coordination proposed in \cite{Farina2018ExAC};
    %
    \item the sequential structure of coordination in our converted game allows the use of the abstraction techniques, as described in Section~\ref{sec:pruning};
    %
    \item our conversion maintains the structure of the original game. This results in a more interpretable tree structure, which is crucial for the design of abstraction techniques;
    %
    \item the auxiliary game of \cite{Farina2018ExAC} uses an initial coordination node with an action for each joint normal-form plan of all team members but one. Instead, our converted game presents nodes with a smaller fanout, thanks to the localized coordination. This makes it feasible to apply \textit{subgame solving} techniques, which proved crucial for the good performance of scalable techniques.
\end{itemize}
%
% Overall, the efficiency enhancements allow us to work in the full converted game, without resorting to \textit{column generation} techniques. The opportunities opened for the use of abstractions and 

% This different expressive power has direct implications on the effect of applying an abstraction \lu{inserire cit} technique.

We can also compare the expressive power of our public-turn-making representation with the original extensive form by considering the effect of (information-lossless/loss) abstractions.

\begin{restatable}{proposition}{propos}
Any action/state abstraction in the original game $\mathcal{G}$ can be mapped specularly in the converted game $\mathcal{G}' = \algoname{ConvertGame} (\mathcal{G})$. The opposite is not true.
\label{th:prop_abs}
\end{restatable}
\begin{proof}
Trivially, any abstraction in the original extensive-form game can be transferred in the public information game by using Algorithm~\ref{alg:PubTeam} directly in the abstracted game.
%
On the other hand, not all abstractions in the public information game can be reflected in the original one.
%
As an example, consider Figure~\ref{fig:simple_example}. If we perform \textit{action abstraction} in the converted game, by collapsing action ''0:A, 1:C'' onto action ''0:A, 1:D'', this abstraction cannot be remapped onto the original game.
This happens because such abstraction corresponds to a constraint on the possible strategies that Player 1 can choose since we are forbidding him to play any pure strategy that requires to play action A at infoset 0 and action C at infoset 1.
%
Such an abstraction does not modify the original game structure, since all A, B, C, D may be played for some specific prescription. 
\end{proof}

Proposition~\ref{th:prop_abs} shows that the converted game is able to encode more information than the original game, suggesting that this higher expressive power could be used to design specific abstraction techniques that also work with the space of players' strategies.

==> content/content-aamas/9_conclusion.tex <==
\section{Conclusions and future work}\label{sec:conclusion}
\raggedbottom
We present a conversion procedure to cast an adversarial team game into a two-player zero-sum game and prove that a Nash Equilibrium in the converted game is strategically equivalent to a TMECor in the original game. This conversion procedure is based on the use of public information among team members, which allows the removal of each player's private information in the converted representation at the cost of an exponential increase in the game size. This tradeoff comes directly from the \textsf{NP}-hardness of the problem of computing a TMECor in a generic team game.
We propose three information-lossless abstraction techniques to obtain a  tree that is more computationally tractable on Kuhn and Leduc poker.
%
Interestingly, our representation is more expressive than the classical extensive-form representation, as we show that any state/action abstraction of the extensive-form game has a counterpart in our conversion, while the reverse does not hold.

%
This conversion retains the public structure of the original game and allows in principle the application of more scalable techniques for solving adversarial team games, such as information-loss abstractions, no-regret learning-based solving algorithms, and subgame solving. We experimentally evaluate the adoption of no-regret learning applied to our converted games, showing that our information-lossless abstractions are not currently sufficient to beat the current state-of-the-art based on column-generation techniques.
%
Hence, the main question that needs to be answered in the future is whether opportune information-lossless abstractions will allow beating column-generation approaches.
%
Nevertheless, our representation provides a direct and clear interpretation of the game when \emph{ex-ante} correlation is used.


%
Furthermore, future works leveraging our techniques in the converted game have therefore the opportunity to overcome current state-of-the-art techniques on larger game instances where an exact solution cannot be found.
%
While the basic and \emph{pruning} algorithms define a conversion procedure that can be used also in an online fashion, the more efficient \emph{folding} conversion does not offer this possibility.
Hence, another direction for future research is the development of a conversion procedure to produce online a folded representation, thus avoiding the cost of constructing the entire tree.
%
Additionally, in principle, our method can be adopted also in $n$ players vs.~$m$ players games. In such scenarios, the support at the equilibrium is no longer small and mathematical programming algorithms lose some efficiency. At the same time, the presence of multiple teams would increase the size of the game tree generated, thus stressing again the importance of the development of suitable and more efficient abstraction techniques. 
%
%Solving team vs team games with a public information approach could therefore be a very interesting future direction. 

==> content/content-aamas/abstract.tex <==
\begin{abstract}


The study of sequential games in which a team plays against an adversary is receiving increasing attention in the scientific literature.
The peculiarity of these games resides in the \emph{asymmetric} information available to the team members during the play which makes the equilibrium computation problem hard even with zero-sum payoffs. The algorithms available in the literature work with implicit representations of the strategy space and mainly resort to \textit{Linear Programming} and \emph{column generation} techniques to enlarge incrementally the strategy space. Such representations prevent the adoption of standard tools such as abstraction generation, game solving, and subgame solving, which demonstrated to be crucial when solving huge, real-world two-player zero-sum games.
Differently from the above works, we answer the question of whether there is any suitable game representation enabling the adoption of those tools.
In particular, our algorithms convert a sequential team game with adversaries to a classical \textit{two-player zero-sum} game. 
In this converted game, the team is transformed into a single coordinator player who only knows information common to the whole team and prescribes to the players an action for any possible private state. Interestingly, we show that our game is more expressive than the original extensive-form game as any state/action abstraction of the extensive-form game can be captured by our representation, while the reverse does not hold.
%We named this procedure \textit{Public Team Conversion}, and it returns an extensive-form game maintaining most of the structure of the original game. 
%Our conversion enables the adoption of highly scalable techniques already available for two-player zero-sum games, including techniques for generating automated abstractions. 
Due to the \textsf{NP}-hard nature of the problem, the resulting Public Team game may be exponentially larger than the original one. To limit this explosion, we provide three algorithms, each returning an \emph{information-lossless abstraction} that dramatically reduces the size of the tree. Most importantly, these abstractions can be produced without generating the original game tree.
% Finally, we present experimental results obtained by applying our techniques to standard benchmarks in the field (\textit{Kuhn} and \textit{Leduc Poker} games) and apply state-of-the-art algorithms for 2p0s games to the resulting game, showing the effectiveness of our approach.
Finally, we show the effectiveness of the proposed approach by presenting experimental results on \textit{Kuhn} and \textit{Leduc Poker} games, obtained by applying state-of-art algorithms for two-player zero-sum games on the converted games. In particular, our information-lossless abstractions allow a reduction of the size of the tree by at least the square root.
\end{abstract}

==> tables/C=3,_A=2,_P1_and_P2_private_state.tex <==
\resizebox{\columnwidth}{!}{%
\begin{tabular}{rrrrr}
\toprule
   $H$ &   normal &    basic &  pruning &  folding \\
\midrule
   1 & 8.00E+00 & 9.00E+00 & 9.00E+00 & 9.00E+00 \\
   2 & 6.40E+01 & 8.10E+01 & 8.10E+01 & 7.50E+01 \\
   3 & 5.12E+02 & 6.57E+02 & 4.05E+02 & 3.75E+02 \\
   4 & 4.10E+03 & 5.26E+03 & 1.56E+03 & 1.46E+03 \\
   5 & 3.28E+04 & 4.21E+04 & 5.16E+03 & 4.86E+03 \\
   6 & 2.62E+05 & 3.37E+05 & 1.55E+04 & 1.48E+04 \\
   7 & 2.10E+06 & 2.70E+06 & 4.37E+04 & 4.18E+04 \\
   8 & 1.68E+07 & 2.16E+07 & 1.17E+05 & 1.13E+05 \\
   9 & 1.34E+08 & 1.73E+08 & 3.04E+05 & 2.93E+05 \\
  10 & 1.07E+09 & 1.38E+09 & 7.65E+05 & 7.40E+05 \\
  11 & 8.59E+09 & 1.10E+10 & 1.88E+06 & 1.82E+06 \\
  12 & 6.87E+10 & 8.84E+10 & 4.53E+06 & 4.41E+06 \\
  13 & 5.50E+11 & 7.07E+11 & 1.08E+07 & 1.05E+07 \\
  14 & 4.40E+12 & 5.65E+12 & 2.52E+07 & 2.46E+07 \\
\bottomrule
\end{tabular}
}

==> tables/C=3,_A=2,_P1_only_private_state.tex <==
\resizebox{\columnwidth}{!}{%
\begin{tabular}{rrrrr}
\toprule
$H$  & normal   & basic    & pruning  & folding  \\
\midrule
1  & 8.00E+00 & 3.00E+00 & 3.00E+00 & 9.00E+00 \\
2  & 6.40E+01 & 2.70E+01 & 2.70E+01 & 7.50E+01 \\
3  & 5.12E+02 & 2.19E+02 & 1.35E+02 & 3.75E+02 \\
4  & 4.10E+03 & 1.76E+03 & 5.19E+02 & 1.46E+03 \\
5  & 3.28E+04 & 1.40E+04 & 1.72E+03 & 4.86E+03 \\
6  & 2.62E+05 & 1.12E+05 & 5.18E+03 & 1.48E+04 \\
7  & 2.10E+06 & 8.99E+05 & 1.46E+04 & 4.18E+04 \\
8  & 1.68E+07 & 7.19E+06 & 3.92E+04 & 1.13E+05 \\
9  & 1.34E+08 & 5.75E+07 & 1.01E+05 & 2.93E+05 \\
10 & 1.07E+09 & 4.60E+08 & 2.55E+05 & 7.40E+05 \\
11 & 8.59E+09 & 3.68E+09 & 6.27E+05 & 1.82E+06 \\
12 & 6.87E+10 & 2.95E+10 & 1.51E+06 & 4.41E+06 \\
13 & 5.50E+11 & 2.36E+11 & 3.59E+06 & 1.05E+07 \\
14 & 4.40E+12 & 1.88E+12 & 8.40E+06 & 2.46E+07 \\
\bottomrule
\end{tabular}
}
